No Identity, no problem: Motion through detection for people tracking

Tracking-by-detection has become the de facto standard approach to people tracking. To increase robustness, some approaches incorporate re-identification using appearance models and regressing motion offset, which requires costly identity annotations. In this paper, we propose exploiting motion clues while providing supervision only for the detections, which is much easier to do. Our algorithm predicts detection heatmaps at two different times, along with a 2D motion estimate between the two images. It then warps one heatmap using the motion estimate and enforces consistency with the other one. This provides the required supervisory signal on the motion without the need for any motion annotations. In this manner, we couple the information obtained from different images during training and increase accuracy, especially in crowded scenes and when using low frame-rate sequences. We show that our approach delivers state-of-the-art results for single- and multi-view multi-target tracking on the MOT17 and WILDTRACK datasets.

==> figs/monocular_drop_fps.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[h]
    \centering
      \includegraphics[width=0.6\linewidth]{images/framerate_sweep_eccv.pdf}
      \caption{\textbf{Tracking results in low FPS scenario.} In low frame rate scenarios our model outperforms the ByteTrack baseline in term of MOTA. The lower the frame rate the higher the performance gap, showing the benefit of the proposed approach.
      }
      \label{fig:low_fps_mota}
    \end{figure}
    

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tabs/ablation.tex <==

\begin{table}[h]
    \begin{center}
    % \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{c c c | c c c c } \toprule
    \multicolumn{3}{c}{Model component} &  \multicolumn{3}{c}{Metrics} \\ 
    Rec. & $L_{\text {se}}$ & $L_{\text {fb}}$ & MODA & L1 & Angle \\ \midrule
    &  &  & 90.7 & 0.87 & 82.0\\
    % \checkmark & & & 90.86 & 79.59 \\
    % &  \checkmark &  & 91.28 & 77.52 \\
    % & & \checkmark & 91.28 & 79.20 \\
    \checkmark & &    & 89.6 & 0.59 & 36.2\\
    \checkmark & \checkmark &  & 90.0 & 0.65 & 43.8 \\
    \checkmark & \checkmark & \checkmark  & 91.8 & 0.58 & 34.8 \\

    \bottomrule
    \end{tabular}
    % }
    \end{center}
    \caption{\textbf{Ablation results on WILDTRACK}  We conduct an ablation study on three components of the system, the spatial extent term (\cref{eq:seLoss}) and the temporal consistency term (\cref{eq:fbLoss}) of the loss function, as well as the removing the reconstruction step (second term of \cref{eq:motLoss}). In terms of MODA, adding the reconstruction loss has detrimental effects, which are balanced out by adding spatial and temporal regularization terms. When considering the motion offset the three components contribute to the quality of the predicted offset. The best results are obtained when the three elements are combined.
    } 
    \label{tab:abla_wild}
    \end{table}

    


==> tabs/detection.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[h]
    \begin{center}
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{5pt}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{r  c c c c c} \toprule
    &  \multicolumn{5}{c}{MultivievX dataset} \\ \cmidrule(lr{.75em}){2-6} 
    model & MOTA & MODA & MODP & Prec. & Rec.  \\ \midrule
    MVDet \cite{hou2020multiview} & - & 83.9 & 79.6 & 96.8 & 86.7 \\
    SHOT \cite{song2021stacked} & - & 88.3 & 82.0 & 96.6 & 91.5 \\
    MVDeTr \cite{hou2021multiview} & - & 93.7 & \textbf{91.3} & \textbf{99.5} & 94.2  \\
    MVAug \cite{Engilberge22a} & - & \textbf{95.3} & 89.7 & 99.4 & 95.9 \\
    Ours & \textbf{81.1} & 94.8 & 88.2 & 99.3 & \textbf{96.0} \\
    \bottomrule
    \end{tabular}
    % }
    \end{center}
    \vspace{-5mm}
      \caption{\textbf{Detection performance on MultiviewX.}  We report MODA, MODP, precision and recall \cite{Kasturi09}. On these detection metrics, our approach performs on par with previous methods, which unfortunately do not report trajectory metrics such as MOTA.}
     \label{tab:sotadetection}
    \end{table}

==> tabs/offset.tex <==
% \begin{table}[h]
%     \begin{center}
%     \renewcommand{\arraystretch}{1.3}
%     \begin{tabular}{r  c c c c c c} \toprule
%     &  \multicolumn{3}{c}{WILDTRACK dataset} & \multicolumn{3}{c}{MultiviewX dataset} \\ 
%     \cmidrule(lr{.75em}){2-4} \cmidrule(lr{.75em}){5-7}
%     model & L1 & Angle & Norm  & L1 & Angle & Norm  \\ \midrule
%     % MVFlow \cite{Engilberge22} & \textbf{93.2} & 79.8 & 96.3 \\
%     RAFT \cite{Teed20a} & 0.61 & 27.87 & 1.18 & 0.61 & 27.87 & 1.18 \\
%     Supervised & 0.59 & 49.6 & 0.57 & 0.61 & 27.87 & 1.18 \\
%     Ours & \textbf{0.36} & \textbf{17.8} & \textbf{0.53} & \textbf{0.36} & \textbf{17.8} & \textbf{0.53} \\
%     \bottomrule
%     \end{tabular}
%     \end{center}
%       \caption{\textbf{Motion offset evaluation} We evaluate 2D motion offset according to three metrics, L1 error, Angular error (in degree) and Norm error. Our model outperforms both baseline by a large margin. Surprisingly, it even performs better than the fully supervised methods, especially in terms of angular error. 
%       }  
%      \label{tab:offset}
%     \end{table}

\begin{table}[t]
  \begin{center}
  \renewcommand{\arraystretch}{1}
  \begin{tabular}{r  c c c} \toprule
  &  \multicolumn{3}{c}{WILDTRACK dataset} \\ 
  \cmidrule(lr{.75em}){2-4}
  model & L1 & Angle & Norm   \\ \midrule
  % MVFlow \cite{Engilberge22} & \textbf{93.2} & 79.8 & 96.3 \\
  RAFT \cite{Teed20a} & 1.06 & 48.8 & 2.07 \\
  Supervised & 0.55 & 32.5 & 0.90\\
  Ours & 0.58 & 34.8 & 0.92 \\
  \bottomrule
  \end{tabular}
  \end{center}
    \caption{\textbf{Motion offset evaluation} We evaluate 2D motion offset according to three metrics, L1 error, Angular error (in degree) and Norm error. Our model outperforms the optical flow baseline by a large margin. It even performs competitively against the fully supervised methods, especially in terms of norm error. 
    }  
   \label{tab:offset}
  \end{table}

==> tabs/tracking_monocular.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table*}[t]
    \begin{center}
    % \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{r c c c c c c } \toprule

        &  \multicolumn{5}{c}{MOT17 val dataset}  \\ \cmidrule(lr{0em}){2-7}
        Model & FPS & Set & MOTA & MOTP & IDF1 & HOTA   \\ \midrule
        
        ByteTrack \cite{ZhangByteTrack2022} & 0.75 & val & 51.1 & 84.6 & 55.0 & 53.5  \\
        Ours & 0.75 & val & - & - & - & -  \\
        \midrule
        ByteTrack \cite{ZhangByteTrack2022} & 2 & val & 59.1 & 84.4 & 59.6 & 56.1  \\
        Ours & 2 & val & - & - & - & -  \\
        \midrule
        ByteTrack \cite{ZhangByteTrack2022} & 30 & val & 77.0 & 84.1 & 77.5 & 66.0 \\
        Ours & 30 & val & - & - & - & - \\
        \midrule
        Ours & 30 & test & 76.5 & 80.8 & 72.4 & 59.8 \\
        
    \bottomrule
    \end{tabular}
    \end{center}
      \caption{\textbf{Tracking performance with low frame rate on MOT17 validation.} We also evaluate our approach in a monocular setting. We use the MOT17 dataset and modify YOLOX and Bytetrack to predict and use motion with the proposed approach.}
     \label{tab:trackingmot}
    \end{table*}

    %Xu, Yuanlu, et al. "Cross-view people tracking by scene-centered spatio-temporal parsing." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 31. No. 1. 2017.

==> tabs/tracking_monocular_reb.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
    \begin{center}
    % \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{r  c c c c } 
        Model & Set & MOTA & HOTA & IDF1    \\ \midrule
        ByteTrack [19]  & val & 76.2 & 65.1 & 75.9 \\
        ByteTrackMotion & val & \textbf{76.4} & \textbf{65.4} & \textbf{76.3} \\
        \midrule
        % ByteTrack [19] \footnote[1]{} & test  & 78.1 & 61.7 & 74.8 \\
        ByteTrackMotion & test & 76.5 & 65.1 & 75.5 \\

    \bottomrule
    \end{tabular}
    \end{center}
    \vspace{-5mm}
      \caption{\textbf{Tracking performance on MOT17 at max FPS}}
     \label{tab:trackingmotreb}
    \vspace{-1.5em}
    \end{table}

    %Xu, Yuanlu, et al. "Cross-view people tracking by scene-centered spatio-temporal parsing." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 31. No. 1. 2017.

==> tabs/tracking_mvx.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[h]
    \begin{center}
    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{r  c c c c c } \toprule

        &  \multicolumn{5}{c}{MultiviewX dataset}  \\ \cmidrule(lr{.75em}){2-6}
        Model & MOTA & MOTP & IDF1 & IDP & IDR   \\ \midrule
        MVFlow \cite{Engilberge22}  & 66.2 & 0.87 & 50.2 & \textbf{56.6} & 45.1 \\
        Ours  & \textbf{81.1} & \textbf{0.55} & \textbf{55.1} & 54.4 & \textbf{55.8} \\
   
    \bottomrule
    \end{tabular}
    \end{center}
      \caption{\textbf{Tracking performance on MultiviewX.} Our model outperforms existing baseline on the metrics related to trajectories by a significant margin. Performance numbers for MVFlow \cite{Engilberge22} was generated from publicly available code.}
     \label{tab:trackingmvx}
    \end{table}

    %Xu, Yuanlu, et al. "Cross-view people tracking by scene-centered spatio-temporal parsing." Proceedings of the AAAI Conference on Artificial Intelligence. Vol. 31. No. 1. 2017.

==> tabs/variable_fps.tex <==

\begin{table}[h]
    \begin{center}
    % \resizebox{\linewidth}{!}{
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{c c | c c } \toprule
    \multicolumn{2}{c}{} &  \multicolumn{2}{c}{Metrics} \\ 
    View aug. & Scene aug.  & MODA & MODP\\ \midrule
    0\% & 0\% & 90.86 & 79.59\\
    25\% & 25\% & 91.49 & 78.24\\
    25\% & 50\% & 90.86 & 79.41\\
    50\% & 25\% & 92.12 & 79.66\\
    50\% & 50\% & \textbf{93.17} & \textbf{79.83}\\
    75\% & 75\% & 90.65 & 78.47\\
    100\% & 100\% & 90.44 & 78.24\\
    \bottomrule
    \end{tabular}
    % }
    \end{center}
    \caption{\textbf{Varying framerate} 
    } 
    \label{tab:prop_wild}
    \end{table} 
